Design and Evaluation of a Hair Combing System Using a General-Purpose Robotic Arm

This work introduces an approach for automatic hair combing by a lightweight robot. For people living with limited mobility, dexterity, or chronic fatigue, combing hair is often a difficult task that negatively impacts personal routines. We propose a modular system for enabling general robot manipulators to assist with a hair-combing task. The system consists of three main components. The first component is the segmentation module, which segments the location of hair in space. The second component is the path planning module that proposes automatically-generated paths through hair based on user input. The final component creates a trajectory for the robot to execute. We quantitatively evaluate the effectiveness of the paths planned by the system with 48 users and qualitatively evaluate the system with 30 users watching videos of the robot performing a hair-combing task in the physical world. The system is shown to effectively comb different hairstyles.

==> figures/content/0-abstract.tex <==
\begin{abstract}
    This work introduces an approach for automatic hair combing by a lightweight robot. For people living with limited mobility, dexterity, or chronic fatigue, combing hair is a difficult task that can negatively impact personal routines. We propose a modular system for enabling general robot manipulators to assist with a hair-combing task. The system consists of three main components.  The first component is the segmentation module, which segments the location of hair in space. The second component is the path planning module that proposes automatically-generated paths through hair based on user input. The final component creates a motion plan for the robot to execute. We quantitatively evaluate the effectiveness of the paths planned by the system and qualitatively evaluate the system with 30 users watching videos of the robot performing a hair-combing task in the physical world. The system is shown to effectively comb different hairstyles.
    
        % \snnote{a system or methodology?} 
        % \snnote{system, methodology or framework? I'd say framework}
    % \snnote{are we checking realism???}
    % This component is evaluated through an online user study, and demonstrates its ability to generate brushstrokes that are able to successfully comb hair. The planning and actuation component generates robot trajectories that follow the paths 
    % % \snnote{trajectories follow the paths?}
    % proposed by the perception component and moves the robot along these trajectories. We evaluate this component through an online user study of videos collected in the real world. 
    
    % Physically assistive robotics enable paralysed patients to perform essential day-to-day activities without the presence of a caregiver. We demonstrate a novel application of robotics in assisted hair brushing. Our vision based system is implemented on the Kinova Gen2 Lightweight robotic arm and designed to perform a full brushing experience with minimal user involvement.
\end{abstract}

==> figures/content/1-Intro.tex <==
\section{Introduction}
% Nine out of ten post-stroke patients experience a form of paralysis, including hemiparesis (weakness on one side of the body), numbness, and problems with balance or coordination [1]. These symptoms severely limit the patient’s ability to perform physical self-care tasks such as bathing and eating that are essential to an individual’s day-to-day life. Traditionally, post-stroke patients require the presence of a caregiver to perform these tasks, but robotics may enable the patient to accomplish the same functions independently. When forgoing a rigorous physical setup,  previous work has shown that a robotic arm may be programmed to assist a user with shaving or wiping [3,4,5].   In our work,  we explore a new application of robotic arm assistance:  hair brushing.  Our system uses a robot arm and a RGB-D camera, to successfully stroke the user’s hair. To plan the brush strokes, we isolate the point cloud of interest from the user’s head with color segmentation and apply an A* algorithm. These strokes are executed by the robot arm as an interpolated trajectory of way points. Our simple system demonstrates robustness to different users with varying hair types.

% SET THE PROBLEM: Talk about mobility issues in people, first prevalence, then costs, then issues with informal caregiving

According to the National Health Interview Survey, there are 40.7 million people in United States living with some form of reduced mobility \cite{nhis_2019} resulting from a variety of factors (e.g., traumatic injury, stroke, genetic causes, etc.). Most items used in activities of daily living (ADLs) are not explicitly designed for people living with reduced mobility and may be completely unusable for them. This requires people living with limited mobility to either purchase specialized items designed for mobility limitations or acquire assistance from others.  However, for many people, neither option may be accessible nor affordable.

The high costs of formal caregivers has necessitated their replacement with family members who give care informally. In 2015, 43.5 million people in the US reported providing informal care in the previous 12 months. Informal caregiving requires providing companionship, personal care, scheduling health services, providing transportation, and more, while at the same time managing one's own job, family finances, household tasks, and other daily activities \cite{feinberg2011valuing}. Due to the increased caregiver load, informal caregiving can be a source of stress and can lead to health problems \cite{pinquart2003differences}. However, assisting people with limited mobility with ADLs is necessary to decrease their risk of depression and, in some forms of limited mobility, can aid in their rehabilitation processes \cite{lin2011does}.

% SHOW BENEFITS OF A POTENTIAL SOLUTION: Talk about how assistive robots can help these people with many daily activities, link it in to how a robot can also help with activities that help with people's sense of autonomy like combing hair. Talk about the benefits of using a multi-purpose system for many tasks vs a specifically designed system for one task

Assistive robots could provide a solution to this growing issue by enabling people with limited mobility to independently perform necessary daily tasks such as eating \cite{bhattacharjee2020more}, drinking \cite{goldau2019autonomous}, and grabbing objects \cite{jain2010assistive}. Areas of self-care such as shaving \cite{hawkins2014assistive}, cleaning \cite{king2010towards}, and dressing \cite{erickson2018deep,kapusta2019personalized} have similarly shown potential for assistive robotics for non-critical tasks. 


% Thus several autonomous or semi-autonomous systems have been developed to assist with ADLs. There are systems aimed to aid with feeding activities \cite{bhattacharjee2020more}, picking items up off of the floor \cite{jain2010assistive}, and handing objects over . There has also been a focus on instrumental activities of daily living (IADLs) which focus on tasks that are not necessary for survival, but are important for functioning in a society. Some examples of these are tasks such as bathing \cite{king2010towards}, dressing \cite{erickson2018deep,kapusta2019personalized}, shaving \cite{hawkins2014assistive}, etc. Recently, there has been a focus on simulating these kinds of tasks to use as a benchmark to evaluate different methods for attempting to solve IADLs \cite{erickson2019assistive}.


% DESCRIBE THE SYSTEM
We propose to expand the abilities of general-purpose assistive robotic arms to the domain of hair-combing, one of the important self-care ADLs. In this work, we provide 
% \snnote{framework; be consistent with the terms}
a minimal system to comb different kinds of hairstyles. The system consists of three modules: an image segmentation module, a path-planning module, and an actuation module.  Together, the system provides users a way to automatically generate paths through their hair and have a robot comb along those paths. The system provides functionality using a
% \snnote{we don't evaluate whether the system gives a sense of autonomy; just say to give more functionality to users with limited mobility}
robotic arm and an RGB-D camera. This work presents a physical implementation of the system on a lightweight Kinova Gen2 robot arm, and an evaluation of its performance. Our results demonstrate that the system successfully combs a variety of hairstyles. 

% \snnote{you should describe the approach and mention what you did, what was the intuition behind and what you found. Also you don't refer to the figure. -- The figure should be a 4x4 (or something) with different users showing the robot performing different strokes, and if possible visualize the robot's paths. Mention also the demo with real users.} 







==> figures/content/2-Background.tex <==
\section{Related Work}

\begin{figure}[t]
  \centering
\includegraphics[width=.9\linewidth]{figures/setup.png}
  \caption{System setup with different hairstyles.}
   \label{fig:setup}
\end{figure}





% According to the National Health Interview Survey, there are 48.7 million people living with some level of reduced mobility due to a wide variety of causes (e.g. traumatic injury, stroke, genetic disposition, etc.) \ndnote{(NHIS, 2018)}. This limited mobility leads to difficulties in performing activities of daily living (ADLs), such as eating, picking items off of the floor, etc. \cite{gill1995assessing}. Because these activities are critical for day-to-day functioning, caretakers are often needed to provide assistance in ADLs for people with reduced mobility.

% Formal caretakers are costly, however, and are often replaced with family members who give care informally. In 2015, 43.5 million Americans reported providing informal care in the past 12 months . Informal care giving requires a family member to provide companionship, personal care, schedule health services, provide transportation, etc. while at the same time managing their own life and jobs, family finances, and performing household tasks \cite{feinberg2011valuing}. Due to the increased load on the caregiver, informal care giving is a major source of stress and can lead to health problems as care continues \cite{pinquart2003differences}. Assisting with ADLs for people with limited mobility can also decrease their risk of depression, and in some cases aid in the rehabilitation process \cite{lin2011does}.

% TALK ABOUT ROBOTS FOR ASSISTANCE
\textit{Assistive Robotics}:
Advances have made it possible to provide robot-assisted ADLs \cite{brose2010role}. Many of the existing systems are high degree-of-freedom arms mounted on tables~\cite{candeias2018vision,jardon2012functional}, wheelchairs~\cite{alqasemi2005wheelchair,hillman2002weston,schrock2009design,gallenberger2019transfer}, or mobile platforms \cite{park2016towards,rhodes2018robot} capable of accomplishing a wide variety of tasks. Several are commercially available \cite{kinova, performance, assistive}.
% \ndnote{(Kinova Robotics, 2020; Performance Health 2020; Assistive Innovations, 2020)}, 
However, these systems are often difficult to control due to the high number of controllable joints, creating a need for some autonomy in order to perform ADLs in an efficient and low-effort manner \cite{herlant2016assistive}. In addition, many of these systems require specialized or wearable sensors that can have unintended negative physical and psychological consequences for the user \cite{schukat2016unintended}. To mitigate those issues, our work aims to be minimally invasive and uses a minimal setup, while additionally utilizing a general-purpose robot arm that is useful in other capacities. 
% \snnote{one novelty of our work is that we use a general-purpose robotic arm, rather than a specialized device. Not sure which of the previous works use a general-purpose arm though}





\textit{Hair Modeling}:
The field of hair modeling focuses on recreating and rendering the entire hair structure in 3D from 2D images \cite{ward2007survey}. 
% Generally, this has two main approaches: directly modeling the orientation field of the hair, or using a data-driven method with 3D exemplars.
In general, hair can be modeled as a collection of curves in 3D space that follow an underlying orientation field that can be inferred from the surface of the hair \cite{saito20183d, zhang2018modeling, zhang2019hair}. Some approaches utilize a database of 3D models, which can be combined to form new styles that are found in single-view images \cite{hu2015single}. Other approaches \cite{chai2012single} use a pipeline for editing hairstyles in portraits by finding orientation fields from images to generate additional strands \cite{chai2012single}. Our system takes inspiration from these works, and models hair as an orientation field. We emphasize being able to generate paths in real time on hair that becomes neater as the system combs it. 
% \snnote{downloading large model is not a problem, I'd say that our system generates paths in real-time that are executed from a real world robotic arm}
% Many of these require interaction in close proximity with the user of the robotic arm, and have employed several safety features concerning motion planning, collision avoidance, and psychological factors \cite{lasota2017survey}. Previous work has also found that the perceived intention of the robot affects how the interactor will perceive the movement of the robot, especially in situations where the robot makes direct contact with the human \cite{chen2011touched}. 


% Building upon these insights, we propose to expand the functionality of robotic arms into the area of autonomous hair-brushing.

==> figures/content/3-SystemDesign.tex <==
\section{System Description}

Our goal is to design a system for people living with limited mobility so they can comb their own hair. 
% We crucially must have a system that is understandable to non-expert users, and allow users to maintain autonomy in their stylistic choices. 
To do this, we propose a system consisting of three modules: the \textit{segmentation module} localizes the hair in space, the \textit{path planning} module proposes brush strokes for the user to select, and the \textit{actuation module} provides the robot with motor commands to move along the user-selected path.


\subsection{Hardware}
The necessary hardware for this system consists of a depth camera and a robot manipulator. Our implementation uses a Microsoft Kinect v1 depth sensor which is commonly used in various robotics domains.  We used the Kinova JACO Gen 2 lightweight robotic manipulator, which is also used effectively in several other assistive domains \cite{maheu2011evaluation, herlant2016assistive} because it is safe for physical interaction. While a comb is also required, our system is designed to work with any comb that can be grasped by the robot arm. We chose a wide-toothed comb, but the comb should be chosen to match the user's hair type. A diagram of the system setup for different hairstyles is shown in Fig. \ref{fig:setup}.
% \snnote{you should also say that the motivation behind using general purpose arm, that can be used for other tasks as well, instead of having a specialized system} 

% The system consists of a JACO 6 Degree-of-Freedom robotic arm, a Kinect camera, and a wide-toothed comb. The camera and arm communicated with each other through ROS and motion planning was performed through the MoveIt library.

\subsection{Segmentation Module}

Hair is difficult to locate in images due to its high variability in color, length, and style. We use a learned approach to segment hair in RGB images and consider this mask a noisy estimate of the hair, We refine this estimate through signal processing techniques as outlined in Fig. \ref{fig:segmentation}

\subsubsection{Segmentation Formulation}

Segmentation is a well-established field of study in computer vision \cite{haralick1985image,ghosh2019understanding}. The overall approach for neural architectures is to take a high dimensional image and learn a low-dimensional representation of the image with an encoder network. The low-dimensional representation is then up-sampled to form an image of the same size as the original image that contains the mask. The loss is quantified as the binary cross-entropy loss between a ground-truth mask and the predicted mask. 
% \snnote{since I think we are using prior work, we should say that we used the approach by...; or is it novel?}:

% \begin{equation}
% \begin{gather}
%     \mathcal{L}(Y,\hat{Y}) = \frac{1}{W \cdot H} \sum_{i=0}^{W-1} \sum_{j=0}^{H-1} Y_{i,j} \cdot \log(\hat{Y}_{i,j}) + (1-Y_{i,j}) \cdot \log(1 - \hat{Y}_{i,j})
% \end{gather}
% \end{equation}
% where $W,H$ are the width and height of the images in pixels, respectively, $Y$ is the ground-truth mask (of size W by H with entries $\in \{0,1\}$), and $\hat{Y}$ is the estimate of the mask (output of the network and also of size W by H with entries $\in [0,1]$). For numerical stability when training, logarithms are clipped to the range $[-100, \infty)$.

Due to the success and efficiency of fine-tuning pre-trained models, we use SqueezeNet \cite{iandola2016squeezenet} as the encoder; it is a small-sized network that achieves high accuracy on Image Net Classification tasks. The smaller model provides comparable accuracy with fewer parameters and thus has a faster run time, which is essential for real-time applications like ours. The decoder has a similar architecture to the encoder, but uses deconvolutional layers instead. We used the Figaro 1k dataset \cite{umar2018hair} for training; it contains a wide variety of labelled hair segments from unconstrained camera angles.

% To make sure that the produced paths are actually on the head of the person, we develop a hair segmentation module. This module defines a bounding box that gives a credible region in which trajectories are expected to occur. We implemented this as pretrained psp-resnet finetuned on the Figaro 1k dataset \cite{umar2018hair} \snnote{this requires an image of the network and a short description of how the network works}. When given an image from a camera, it returns a mask of pixels that are likely to be the hair. 
\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{figures/segmentation.png}
  \caption{Diagram of the image segmentation module.}
   \label{fig:segmentation}
\end{figure}

\subsubsection{Refining the segmented region}

% \snnote{why do we need a bounded box? you need to explain the system parts better}
To improve the fidelity of the mask, we extract the points in XYZ space that correspond with the hair pixels. Two main sources of error are of concern in accurately segmenting hair from RGB images: \textit{temporal} errors and \textit{spatial} errors. 

Temporal errors can result from sensor noise, causing the estimated hair mask to form discontinuities or disappear completely for a single frame. 
% \snnote{I dont understand the sentence}
To reduce the impact of such high-frequency noise, we use an exponential smoothing filter to average values from the stream of masks. This filter averages masks over time, but gives exponentially higher weights to images nearby in the sequence. This reduces the effects of high-frequency noise (i.e., sensor noise) but allows low-frequency patterns (i.e., user movement) to pass through. 
% \snnote{why do you do that?}. 
The filter is described by the following iterative function:

\begin{equation}
mask(t, \hat{Y}_t) = \left\{
        \begin{array}{ll}
            \hat{Y}_t & \quad t = 0 \\
            \alpha \cdot \hat{Y}_{t} + (1-\alpha) \cdot mask(t-1, \hat{Y}_{t-1}) & \quad t > 0
        \end{array}
        \right\}
\end{equation}

where $t$ is the timestep, $\hat{Y}_t$ is the output of the segmentation network for frame , and $\alpha$ is the smoothing parameter. Higher values of $\alpha$ allow better tracking of user movement and lower values reduce the effect of sensor noise. Our system uses $\alpha=0.9$.

To address spatial errors (i.e., false-positives, other people in the frame, etc.) we first select the largest contiguous area in the mask. We then find the median value of pixels selected as representing the depth of the hair,  an estimate that is robust to outliers. Points that are within two standard deviations of this median value and have hues within the range of the pixels in the mask are added to the mask to reduce the number of false negatives.

% We then remove outliers by selecting the inter-quartile range of depth values associated with the pixels, that trims errors that come from pixels that are false positives, as well as pixels that are failures of the sensor. The variability of depth that provides the credible boundary of the hair is set as plus or minus two standard deviations.
% \snnote{I don't understand which part is done automatically and which part is done by the user}.

% By Chebyshev's inequality, two standard deviations will contain at least 75% of the hair points in the hair for arbitrary distributions. 


\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/processingpipelinearrows.png}
  \caption{Overview of path-planning module.}
   \label{pathplanningpipeline}
\end{figure}

\subsection{Path Planning Module}

We developed a path planning module that takes a user-specified point as input and produces a path through the hair that aligns with the natural curvature of the hair. Following works from Computer Graphics on hair rendering, we model the flow of hair as a differential field \cite{chai2012single}. To obtain the differential field, we find the orientation of the hair in the image.
We consider a path that follows the flow of the hair as a solution to the differential field with initial conditions defined as the point a user selects as the path's starting point.
% Then a path that follows the flow of the hair is calculated as a particular solution with the user's selected point as the initial condition, we use Euler integration \snnote{I am not sure what you mean here} to find a particular solution to the differential field, a path that follows the natural flow of the hair, beginning at a user-selected point.
For the following sections, we leverage the common assumption that an image is a smooth continuous function that maps XY coordinates to intensity values. The function is discretized into pixels and the intensity value at each pixel is noisily sampled from the underlying intensity function. This assumption allows us to take derivatives over the image to construct the orientation field.

% The second method uses the RGB image from the Kinect camera to directly draw a path that follows the natural flows of the hair in the image. To do this we exaggerate the flows of the hair using a coherence-enhancing shock filter \cite{weickert2003coherence}. The intuition of this filter is that it erodes the image where the laplacian of the image is positive and dilates the image where the laplacian of the image is negative \snnote{why does the Laplacian matter?}. This effectively smooths the image in directions along parallel structures and sharpens the image in directions orthogonal to parallel structures.

\subsubsection{Coherence-Enhancing Shock Filters} 

We first use the method described by Weickert et al. \cite{weickert2003coherence} to make the natural flows of the hair more coherent, reducing the effect that stray strands of hair may have on the calculation of orientation. To do this, we iteratively refine an image by increasing contrast in the direction of the greatest change of the intensity gradient (directions perpendicular to the flow of hair), and decreasing contrast in the direction of the lowest change of the intensity gradient. 

First, eigenvectors are calculated for each pixel's local neighborhood, providing the direction of greatest change in intensity. 
The convexity of the image at the pixel's location is calculated by the second derivative in the direction of the dominant eigenvector is calculated.
If the second derivative is positive, the intensity function is concave up, and we want to make the point more intense to match its surroundings. If the second derivative is negative, we want to make the point less intense to match its surroundings. The net effect of this process is to increase the contrast in the direction of the greatest change in intensity. The process is shown in Algorithm \ref{shockFilter}, and the effect on images is seen in Fig. \ref{pathplanningpipeline}.




% This is formulated as an image modeled as a discretization of a continuous function that maps pixels to an intensity value $f: \mathbb{R}^2 \rightarrow \mathbb{R}$ \snnote{I am not sure what this means}. The function is then evolved according to the following partial differential equation:

% \begin{equation}
% \begin{gathered}
%     u_t = -sign(u_{ww})*|\Delta u|\\
%     \text{with initial condition } u(x,y,0) = f(x,y)\\
%     \text{and } u_{ww} =  e1_{x}^2*u_{xx} + 2*e1_x*e1_y*u_{xy} + e1_y^2*u_{yy} 
% \end{gathered}
% \end{equation}

% Where w is the dominant eigenvector. $u_ww$ is positive when the pixel in question is a minimum in the direction of the dominant eigenvector, the above equation simplifies to $u_t = -|\Delta u|$ which is the definition of an erosion process. When the pixel in question is a maximum, the equation simplifies to $u_t = -|\Delta u|$, which is a dilation process. \snnote{what is the intuition behind this equation?}

\begin{algorithm}
\caption{Coherence Filter}\label{shockFilter}
\begin{algorithmic}[1]
\State \textbf{Input:} Image $I$, kernel size $K_\delta$ for approximating derivative, kernel size $K_e$ for calculating eigen vectors,kernel size $K_m$ for calculating mx  and min values, Constant $C_{blend}$ the blending rate for each iteration, and $T$ the total number of iterations.

% \State $\Sigma_s, \Sigma_e,C_{blend}, iterations \gets \text{11, 11, 0.5, 4}$
% \State $\textit{image} \gets \text{input RGB image}$
\For{t=1,2,..T}
        \State calculate first (normalized) eigenvector $[e_x,e_y]$ for each sub image of size $K_e \times K_e$ in $I_t$
        \State Approximate $\frac{\delta^2 I}{\delta x^2}$, $\frac{\delta^2 I}{\delta x\delta y}$, and $\frac{\delta^2 I}{\delta y^2}$ with a sobel filter of size $K_\delta$.
        \State Compute  $I_{vv}: e_x^2*\frac{\delta^2 I}{\delta x^2} +2*e_x*e_y*\frac{\delta^2 I}{\delta x\delta y} + e_y^2*\frac{\delta^2 I}{\delta y^2}$
        % \State $g_{vv} \gets x^2*g_{xx} +2*x*y*g_{xy} + y^2*g_{yy}$ \snnote{what is this doing?}
        % \State $erode,dilate \gets erode(image),dilate(image)$ \snnote{is this eroded / dilated images?}
        \State Create a new image $I_t'$, where for each sub image of size of size $K_m \times K_m$ in $I$, we take the maximum value if $I_{vv} > 0$ and the minimum if $I_{vv} < 0$ 
        % \State $toBlend \gets erode[g_{vv}>0] + dilate[g_{vv}<0]$
        \State $I_{t+1} \gets I_t*C_{blend} + I_t'*(1-C_{blend})$
      \EndFor
\State \textbf{return} \text{image}
\State \textit{Note: our implementation uses $K_{\delta}=7$, $K_{e}=11$, \Statex  $K_m=3$, $C_{blend}=0.9$, and $T=3$}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Find Orientations}\label{GST}
\begin{algorithmic}[1]
\State \textbf{Input:} Image $I$, kernel size $K_\delta$ for approximating derivative, kernel size $K_E$ for approximating expectation

\State Approximate $\frac{\delta I}{\delta x}$ and $\frac{\delta I}{\delta y}$ (with a sobel filter of size $K_\delta$).
\State Construct:
$\begin{bmatrix}
I_xI_x & I_xI_y \\
I_yI_x & I_yI_y 
\end{bmatrix} = \nabla I^T \nabla I = S_0$ 
% \snnote{is this equal to Eq.(2)? If yes, you should state that. If not, it should be clear how Eq.(2) relates to the algorithm}
\State Locally average each element in $S_0$ with kernel size $K_E$ to calculate Structure Tensor: $\begin{bmatrix}
J_{11} & J_{12} \\
J_{21} & J_{22} 
\end{bmatrix} = S_{K_E}$

\State Calculate local orientation: $\Theta = \frac{1}{2} atan2(\frac{J_{12} + J{21}}{J_{22} - J{11}}) + \frac{\pi}{2}$

% \State $\Sigma_s, \Sigma_b \gets \text{3, 5}$
% \State $\textit{image} \gets \text{input image}$
% \State $g_{x} \gets sobel(\text{image, dx=1, dy=0, size=}\Sigma_s)$
% \State $g_{y} \gets sobel(\text{image, dx=0, dy=1, size=}\Sigma_s)$
% \State $g_{x}^2 \gets elementMultiply(g_{x},g_{x})$
% \State $g_{y}^2 \gets elementMultiply(g_{y},g_{y})$
% \State $g_{x}g_{y} \gets elementMultiply(g_{x},g_{y})$

% \State $J_{11} \gets boxFilter(g_{x}^2, size=\Sigma_b)$
% \State $J_{12} = J_{21} \gets boxFilter(g_{x}g_{y}, size=\Sigma_b)$
% \State $J_{22} \gets boxFilter(g_{y}^2, size=\Sigma_b)$
% \State $orientations \gets 0.5 * phase(J_{22} - J_{11}, J_{12}*J_{21})$

\State \textbf{return} $\Theta$
\State \textit{Note: our implementation uses $K_{\delta}=3$ and $K_{E}=5$}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Calculate Path}\label{Path}
\begin{algorithmic}[1]
\State \textbf{Input:} Orientation image $\Theta$, selected pixel for the start of the path $v_0 = [v_x,v_y]$, step size $k$ (in pixels).
\State initialize $path$ with $v_0$
% \State $\textit{input} \gets \text{RGB image}$
% \State $\textit{image} \gets \text{Coherence Filter Image}(input)$
% \State $\textit{orientations} \gets \text{Calculate Orientations}(image)$
% \State $point \gets \text{clicked point in image}$
% \State $path \gets emptyList$
\While {$v_t$ is within bounds of hair}
\State $\theta_{v_t} = \Theta[v_t]$
\State $v_{t+1} \gets v_t + k \cdot [cos(\theta_{v_t}), sin(\theta_{v_t})]$
\State append $v_{t+1}$ to the path
% \State $direction \gets orientations[point]$
% \State $point \gets point + length * rotation(direction)$ \snnote{not sure what this equation means}
\EndWhile

\State \textbf{return} $path$

\State \textit{Note: our implementation uses $k=6$}
\end{algorithmic}
\end{algorithm}










\subsubsection{Calculating Orientation}
Once the image has been filtered to enhance the coherence of the hair flows, the next step is to calculate the direction of the hair flows in the image. This is achieved from the gradient structure tensor, which is defined continuously for a point $p$ as:

\begin{gather}
   S_w(p) = \begin{bmatrix}
    \int_r w(r) \cdot (I_x(p-r))^2 & \int_r w(r) \cdot I_x(p-r)I_y(p-r) \\
    \int_r w(r) \cdot I_y(p-r)I_x(p-r)& \int_r w(r) \cdot (I_y(p-r))^2 
    \end{bmatrix}
\end{gather}

where $w$ represents a window of the part of the image to consider. The integral corresponds to the convolution operation over a continuous image. The pseudo-code for computing $S_w$ discretely for all pixels is detailed in Algorithm \ref{GST} on lines 2-4. Orientations from this structure tensor following the equation on line 5, as detailed by Yang \cite{yang1996structure}.


\subsubsection{Generating the path}

Once the orientation field is constructed, the user selects a point on the image for the starting point for the comb. Then the path is iteratively generated by adding new points that follow the direction of the orientation field, as described in Algorithm \ref{Path}.

\subsection{Actuation Module}

The actuation module takes in the path in the form of pixel coordinates and maps them to task-space poses.  The XYZ position of the pose comes from the point in the pointcloud that is indexed by the pixel in the path.
% \snnote{say that they are mapped to task space poses, then say how the XYZ and orientations are defined} XYZ coordinates using the RGB-D camera.
Orientations are assigned to each point so as to have the teeth of the comb (z-axis of end effector, following the Denavit–Hartenberg convention) point orthogonally into the user's hair plane $H$. $H$ represents the plane formed by the visible portion of the hair and is defined by the normal vector $\vec{h}$.
% \snnote{this needs a figure or reference to a figure}. 
The Y axis of the end effector is aligned with the vector tangent to the path that the robot is following, projected onto the hair plane. This is approximated with the centered difference of the previous and next points in the path. Figure~\ref{fig:geometrySetup} shows this graphically, where the unit axes of the end effector's coordinate frame (measured from the camera's reference frame) at point $p_t$ are given by:
% \snnote{should be $\vec{p}_{t-1}$ instead of  $\vec{p_{t-1}}$} 

\begin{gather}
EE_x = EE_y \times EE_z\\
EE_y = \frac{(\vec{p}_{t-1} - \vec{p}_{t+1}) - [(\vec{p}_{t-1} - \vec{p}_{t+1}) \cdot \vec{h}]\vec{h}}{\left\Vert  (\vec{p}_{t-1} - \vec{p}_{t+1}) - [(\vec{p}_{t-1} - \vec{p}_{t+1}) \cdot \vec{h}]\vec{h}  \right\Vert}\\
EE_z = \vec{h} 
\end{gather}

A motion plan for the robot end effector is planned in task space, following joint velocity and acceleration constraints. A preview of the resulting motion plan is shown to the user. If the user accepts the preview, the robot executes the motion plan, otherwise the system prompts the user to select a new point in the hair and generates a new path and trajectory. 
% \snnote{see Maja's comment: what happens if the user does not accept?}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/geometryDiagram.png}
  \caption{Creating task-space poses from points of stroke.}
   \label{fig:geometrySetup}
\end{figure}



% Once the points generated by the algorithm that are likely to be hair are determined, the desired trajectory is determined in SE(3) space by enforcing the constraints that the z-axis of the end-effector will by orthogonal to the local plane of the hair, fixing the rotations about the x and y axes. We additionally enforce that the rotation about the z axis of the end-effector is such that the comb is always perpendicular to the direction of motion. \snnote{this needs a picture -- we also have not spoken about any robots} This is approximated as the average of the forward and backward derivatives for successive points in the trajectory \snnote{what are the forward and backward derivatives?}.
























% \section{Perception Module}

% To plan trajectories through the hair, we developed two methodologies: a mesh-based method which creates a 3D representation of the user's hair and uses this representation to plan through the hair  \snnote{also write about how you use the mesh}, and an image-based method which generates a path from the image of the user's hair \snnote{also write how you follow the image}.



% \subsection{Image-Based Method}
% % The second method uses the RGB image from the Kinect camera to directly draw a path that follows the natural flows of the hair in the image. To do this we exaggerate the flows of the hair using a coherence-enhancing shock filter \cite{weickert2003coherence}. This filter takes an image \textit{i} which is a section of the original image and calculates the second-moment matrix of the image i, which is defined as 
% % $$
% % \begin{bmatrix} 
% % J_{xx} & J_{xy} \\
% % J_{yx} & J_{yy} \\
% % \end{bmatrix}
% % \quad
% % $$
% % The values of these derivatives are discretely approximated with a sobel filter. The second moment matrix is then decomposed into its eigen vectors, where $\lambda_1, \lambda_2$ represent the eigenvalues of their corresponding vectors. In the case when an image has a clear directionality, $\lambda_1 >> \lambda_2$, and the eigenvector corresponding to $\lambda_1$ points in the direction of the greatest change in the image. In the case where  $\lambda_1 \approx \lambda_2$, there is no clear structure in the image. The image then eroded and dilated in the directions orthogonal to the first eigen vector to preserve the directional structure of the image. The contrast is minimized in the direction orthogonal to the first eigen vector and is maximized in the direction of the first eigen vector. The strength of this sharpening is proportional to the relative weights of $\lambda_1$ and $\lambda_2$

% % To plan the paths, the coherence-enhanced image is used. We calculate the second -moment matrix again, and instead of eroding and dilating in the direction of the largest eigen vector, we create a new image of orientations from the these vectors, represented as angles. Then, a user selects one part of the image to start planning a path at. The angle information is treated as a differential field, and Euler integration is used to find a path that traverses the hair: starting with the first pixel, we take a small step in the direction of the angle specified from the image of angles and use this as the beginning for the next step of the path. This continues until the path reaches the end of the hair, which can be determined by both lower coherence of the image ($\lambda_1 \approx \lambda_2$), or the depth of the image at the new point is much higher than the previous points on the image.






% \begin{figure}[htb]
%     \centering
%     \begin{subfigure}{0.16\textwidth}
%       \includegraphics[width=\linewidth]{figures/ply_path.png}
%       \caption{A* Path}
%     \end{subfigure}\hfil
%     \begin{subfigure}{0.16\textwidth}
%       \includegraphics[width=\linewidth]{figures/gst_path.png}
%       \caption{GST Path}
%     \end{subfigure}\hfil
%     \begin{subfigure}{0.16\textwidth}
%       \includegraphics[width=\linewidth]{figures/human_path.png}
%       \caption{Human Path}
%     \end{subfigure}\hfil
%     \caption{A comparison of the three path types drawn on the same hairstyle. \snnote{need better example for human paths}}
%     \label{pathstyles}
% \end{figure}    

% \subsection{Moving the Arm}
% Once the trajectory is defined in the task space, the robot must plan a movement that achieves the points in the task space. This can be accomplished by any task-space planning algorithm. Our implementation uses the MoveIt! framework, and the Open Motion Planning Library and inverse kinematics solver for the JACO2 arm that is provided by KINOVA robotics. This, however, can be swapped out for any combination of motion planning library or arm that is desired to be used, as the generation of the paths are independent of the robot's actual movement. The overall flow of the entire system is shown in Figure \ref{fig:systemDiagram}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/diagram.png}
%   \caption{Block diagram of the system. \snnote{the block diagram needs to have pictures, see }}
%   \label{fig:systemDiagram}
% \end{figure}

% \subsubsection{Interaction}
% The interaction loop consists of three main steps. First, the user is presented with a live video feed of their hair and they are asked to select a point on their head that they would like to start combing. The path planning algorithm then generates a proposed path and asks the user for their feedback. If the user agrees that the path is appropriate for their hairstyle, the robot will then demonstrate its trajectory in simulation to show the user how it will move. If the user agrees to the movement of the arm, the robot executes the stroke. If there is any stage at which the user disagrees with the movement of the arm, the interaction starts again. This process is repeated until the user is satisfied with the way that their hair looks \snnote{how does the user rate their agreement / disagreement? Also how does that work with the online study?}.

==> figures/content/4-PathPlanning.tex <==

\begin{figure*}[t]
    \centering
    
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/002.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/012.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/037.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/056.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/093.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/150.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/223.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/249.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/272.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/381.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    
    \medskip
    
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/054.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/060.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/086.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/087.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/137.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/171.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/234.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/289.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/332.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/429.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added

    
    \medskip
    
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/221.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/423.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/335.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/303.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/212.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/188.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/159.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/142.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/109.png}
      % \caption{image1}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.095\textwidth}
      \includegraphics[width=\linewidth]{figures/path_styles/017.png}
      % \caption{image1}
    \end{subfigure}\hfil % <-- added
    \label{hairstyles}
    \caption{Examples of generated paths on the thirty hairstyles from one of three camera viewpoints used to evaluate the algorithms in the user study. Each hairstyle also came in five different colors. Red paths represent the mesh-based method, orange paths represent the image-based method, and blue paths represent the human-drawn paths.
    % \snnote{we need to show different paths per hair style, maybe different colors for each algorithm}
    }
    \vspace{-0.3cm}
\end{figure*}


\section{Path Planning Evaluation}
% To better evaluate the path-planning module, we propose a baseline alternative, where the assumption is that users \textit{do not} have a strong preference for the robot to follow the natural flow of their hair, and instead desire the robot to brush directly downward following the shortest path from the top of their hair to the bottom of their hair \snnote{we haven't said anything about user preferences; instead just mention the baseline}.
To evaluate the path planning module, we propose a baseline alternative, where the appropriate path to comb hair is the shortest path from the top of the hair to the bottom of the hair. 
% \snnote{isn't it the bottom of the mesh?}

\subsection{Baseline Method}
To create paths that move directly downward, we plan directly on a mesh created from the point cloud of the hair, taken by the Kinect camera. Next we segment the image based on color and depth to find candidate point clouds of the head. A human operator selects the subset of point clouds that correspond to the user's hair. The union of these point clouds represent the entirety of the hair structure to be brushed. The resulting point cloud is then converted to a mesh by using a greedy surface triangulation algorithm \cite{Marton09ICRA} from the PointCloud Library \cite{Rusu_ICRA2011_PCL}. The mesh and generated paths are shown in Fig. \ref{fig:meshPaths}.
% \snnote{this needs pictures}
% \ndnote{I don't know the details about how the PCL algorithm works, but I think that there are several algorithms that convert point clouds to meshes...I would assume that the PCL one is called the Pivoting Ball Algorithm, but I don't know if I should explain more about that or not}
Once the mesh is created, paths are formed by sampling mesh vertices from the upper portion of the hair mesh model. The mesh is considered a graph with nodes corresponding to mesh vertices and edges corresponding to the edges of the triangles that define the mesh. We define the goal as any point in the bottom portion of the hair mesh. We then formulate path planning as finding a low-cost path from the start vertex to one of the vertices in the goal set. For simplicity and speed, we find these paths using the A* algorithm \cite{russell2002artificial} with Euclidean distance as the distance metric, and the straight-line distance to the bottom of the mesh as the heuristic.
% \snnote{why the upper tenth}? 
% and finding paths through the A* algorithm. 
% \snnote{why the A*?}


% This is accomplished \snnote{please use active voice} by considering the mesh as a graph in which the mesh vertices are the nodes, and the triangles are the edges between nodes. Expanding a node returns the other nodes that are connected to the original node by at least one triangle \snnote{I am not sure what this means}. There are then two other metrics that are needed to perform A*: distance of a node from the start (G(x)) and a heuristic to the end (H(x)). The distance is calculated using the euclidean distance (L2 norm) between the points. The Heuristic we use is y-axis distance to the lower x-z plane formed by the bounding box of the hair mesh \snnote{why is that?}. Instead of having one goal node, we have a set of goal nodes which are acceptable terminal locations. This set is defined as the set of all points in the lower tenth of the hair mesh model.

To generate a variety of paths, the algorithm is run several times using sampled start states from the upper portion of the hair. The paths with the lowest overall distances are selected as the set of brush strokes to show in the study.
% \snnote{in the future we may want to consider having the operator select the starting point for fairer comparison} 
% \snnote{we need a picture with the paths and the path selected}

\begin{figure}[h]
  \centering
%   \includegraphics[width=\linewidth]{figures/meshPaths.png}
   \begin{subfigure}{0.5\linewidth}
   \centering
      \includegraphics[width=.73\linewidth]{figures/hairpointcloud.png}
       \caption{Pointcloud data from Kinect.}
    
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.5\linewidth}
    \centering
      \includegraphics[width=.73\linewidth]{figures/meshwithpaths.png}
       \caption{Output mesh with trajectories.}
    
    \end{subfigure}\hfil % <-- added
    
  \caption{Example paths generated by the mesh-based method.}
   \label{fig:meshPaths}
   \vspace{-0.6cm}
\end{figure}


\subsection{Study Setup}
To evaluate the strengths and weaknesses of the three approaches, we measured user perception of the methods through an on-line study using Amazon Mechanical Turk. A variety of hairstyles were selected from the USC hair salon database \cite{hu2015single}. Ten short, ten medium, and ten long hairstyles were selected at random, and rendered in one of five hair colors (black, brown, auburn, blond(e), and grey) from one of three camera angles.  

Each MTurk participant saw 10 of the 30 hairstyles at random, and was shown three algorithms for generating paths: the mesh-based method (baseline), the image-based method (proposed method), and a set of human-drawn paths as a high-quality reference point. Human-drawn paths were generated by an independent researcher not affiliated with the project.
% \snnote{why did you choose the set of human-drawn paths} 
For each algorithm, participants were shown three paths to provide a holistic view of the types of paths the algorithms generated. For each algorithm, participants rated the generated paths on: 1) whether the paths \textit{are able} to brush hair, and 2) whether the paths \textit{effectively} brush the hair. 
% \snnote{questionnaire should be on a table} 
% Finally, we presented three random paths, one from each algorithm, and asked the participants to choose the path that they believed would be the best of the three choices for brushing the hair.
% \snnote{you mean one of the three paths?}. 


% \begin{table}[h]
%   \centering
%   \begin{tabular}{ |c c| }
% \hline
%  Measurement & Question\\ 
%  \hline
%  Completeness & ...be able to brush the hair\\  
%  Effectiveness &  ...effectively brush the hair\\
%  Effectiveness & ...ineffectively brush the hair\\
%  \hline
% \end{tabular}
%   \caption{Questions posed to participants. Questions were prefaced with "From the paths shown above, a brush moving along these paths would..."}
%   \label{tab:questions}
% \end{table}

\subsection{Hypotheses}
\noindent
\textbf{H1}: \textit{Participants will prefer paths that vary in their start point rather than paths that always start at the top, and thus rate the image-based method as generating paths that are more complete than the mesh-based method.} 

% \snnote{what are the image-based, and mesh-based methods? If you use these terms, you should say this explicitly when describing the study}
% \snnote{hypothesis requires some explanation why you consider it. Also, what's the GST method?}\\
\noindent
\textbf{H2}: \textit{Participants will prefer paths that follow the flow of the hair, and thus rate the image-based method as generating paths that are more effective than the mesh-based method.}\\ 
% \snnote{what do you mean more optimal? Either they're optimal or not}}\\



\subsection{Results}
The study received 48 respondents (27 women, 21 men; median age range 25-34). Responses were measured on a scale of -3 to 3, with 0 indicating neutral responses. A repeated-measures ANOVA test found significant differences for the main effect of algorithm on reported \textbf{completeness} of planned path, with F(2,94) = 24.12, $p<.001$. Pairwise t-tests were used for post-hoc analysis, revealing that all pairwise comparisons were significant after Bonferroni correction. The mesh-based method of planning paths (M=.99) received significantly lower ratings than the image-based method (M=1.53), $p<.001$, $\eta^2=.09$ which was in turn rated as less complete than the human-drawn paths (M=1.70), $p=.01$, $\eta^2=.01$. The difference between the mesh-based method and the human-drawn paths was also significant, $p<.001$, $\eta^2=.17$. This supports \textbf{H1}.


We performed the same analysis for \textbf{effectiveness} ratings. A repeated-measures ANOVA test shows significant differences by algorithm type, with F(2,94) = 21.69, $p<.001$. Pairwise t-tests show significance between all comparisons with $p<.001$, where the mesh-based method (M=.32) was lower than the image-based method (M=.89), $\eta^2=.08$, and the human-drawn paths (M=1.22) were rated the highest, $\eta^2=.04$. This supports \textbf{H2}.

Qualitative notes from participants in the study revealed that they found the human paths to be rated the most highly because they tended to "follow the hair flow", but were also "long and straight". The main concern with the image-based method was the it followed the path of the hair too closely. This is evident for the hairstyles that have waves, where combing in a wavy path may be inefficient. Because the hair can deform as the comb passes through it, moving along the waves is less direct than moving straight.
% \snnote{Generated paths need to be discussed. How are they different? What can be improved?}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/PathEvals.pdf}
  \caption{Means of the three different algorithms. Error bars represent 95\% Confidence Intervals of mean ratings.}
   \label{fig:Evaluations}
   
\end{figure}




% \subsection{Qualitative Insights}



















==> figures/content/5-Movement.tex <==
\section{Trajectory Execution}

\begin{table*}[t]
  \begin{centering}
  \begin{tabular}{ |c c c| }
\hline
 Theme & Positive Example & Negative Example \\ 
 \hline
 Effectiveness & "...the hair [that] the robot worked on looked much better..." & "...there is no effect on the hair that the robot is combing." \\  
 Force & "It did seem gentle though, so that is good." & "...it looked like it was pushing rather rough at the hair." \\
 Movement & "This robot appeared to have finesse and sensitive movements." & "...there is no grace or nuance to the motion." \\
 \hline
\end{tabular}
  \caption{Examples of positive and negative qualitative responses from participants for each theme.}
  \label{tab:responses}
  \end{centering}
  \vspace{-0.3cm}
\end{table*}


\subsection{On-line User Study}
To evaluate the performance of the physical robot implementation of the system, we recorded three videos of the robot combing three different wigs. The wigs were of different colors and hairstyles and were representative samples of the hairstyles in the first study, consisting of a short brown wig, a medium-length pink wig, and a long blonde wig. The wigs were teased so that the hair was in a state that would warrant using a hair-combing device. Each video showed the wig and robot arm from the side so that study participants could see both the end effector and wig at all times, shown in Fig. \ref{fig:studyFrame}. We used a plain white background for all videos. A human operator operated the robot system off-screen. The participants watched the wig being combed by the robot, where the first and final strokes were filmed in real time and the middle strokes were filmed at 20x speed to show the progress that the robot makes over the course of the hair-combing interaction. Participants were then asked to rate the effectiveness of the combing as well as their level of comfort with using the system. The participants were also asked to justify their reasoning.    

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/frames.png}
  \caption{Sample frames of the video shown to the participants.}
   \label{fig:studyFrame}
   \vspace{-0.5cm}
\end{figure}
% \subsection{Hypotheses}
% \noindent
% \textbf{H1}: \textit{Participants will rate the robotic hair combing interaction as effective.}\\
% \textbf{H2}: \textit{Participants would be comfortable with using the robot to comb their own hair.}\\

% \subsection{Quantitative Analysis}
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/HairResponses.pdf}
%   \caption{Means of the three different algorithms. Error bars represent 95\% Confidence Intervals of mean ratings.}
%   \label{fig:hairBarGraph}
% \end{figure}

% The study received 30 responses (17 men, 13 women; median age range 25-34). A T-test was used to determine differences of ratings for each hair style in terms of effectiveness and the participants' comfort level with using the robot themselves. A repeated measures ANOVA reveals that participants provided different ratings for both effectiveness and comfort based on the hair style that the rated, indicating that analysis must be done on each style separately. Regarding effectiveness, a two-sided t-test reveals that only the medium pink hair was rated as being effectively brushed (M=.97), $p=.003$. While positive, the effectiveness ratings of the blonde hair (M=.60), $p=.150$ were not significant. The effectiveness ratings for the short brown hair (M=-  1.00), $p=.011$, however, were rated as significantly ineffective. This provides very limited support for \textbf{H1} for certain hairstyles.

% In terms of comfort, two-sided T-tests shows that the participants were generally \textit{uncomfortable} with the idea of a robot combing their hair when viewing the robot combing the short brown hair (M=-1.26), $p=.009$. The other two hair styles received negative ratings overall, but were not significant. The medium pink hair (M=-.30), while rated the highest in effectiveness had a slightly lower mean than the long blonde hair (M=-.13). This does not support \textbf{H2}.

\subsection{Qualitative Analysis}
The study received 30 responses (17 men, 13 women; median age range 25-34). We conducted a qualitative analysis of the open-ended survey responses, and utilized a grounded-theory approach \cite{heath2004developing} where we categorized responses by theme in a data-driven manner. 
% We then go back through the responses and then assign them to the different themes we developed. This process is iteratively repeated until the responses can be accurately sorted into respective categories. We then evaluate that these responses are consistent with responses of held-out participants to make sure that our coding scheme accurately represents the constructs that were at play during the evaluation of the system. 
% \snnote{if you mnention this approach, you should have a table with assigned responses for each theme.}
The qualitative analysis revealed three main themes in participants' evaluations of the system. The first theme was related to the effectiveness of the task of hair combing. The second theme was the perception of the amount of force that was used throughout the interaction.  The third theme was related to how the robot moved while combing hair. Representative positive and negative examples of each theme are shown in Table~\ref{tab:responses}.

\subsubsection{Effectiveness}
The theme of effectiveness had several subcomponents. The top three were: final alignment of hair, depth of combing, and time it takes the robot to comb.

The final alignment of the hair was mentioned in 31 of the 90 responses; 25 of these responses indicated that respondents thought that the hair ended up "...straighter than before it started combing" or some variant mentioning that the hair looked neater after the combing interaction. This subcomponent received the highest number of positive mentions across all categories. 
% The other six responses reported that they were not able see a difference before or after combing. 
% \snnote{new paragraph}

Related to depth of combing, the majority of negative responses came from the short brown hairstyle. 19 participants mentioned that the robot appears to comb the hair superficially, but 4 of the responses indicate that the robot penetrates the deeper layers of the hair. All 4 positive responses were for the medium and long hairstyles. 

The subcomponent of timing was noted in 24 responses. 19 of these responses indicated that the robot took too long to move when combing, negatively affecting the interaction. Interestingly, 4 responses positively described the slow movement of the robot as cautious and gentle.
% One of the other two responses indicated that the robot was able to quickly brush the hair, and the other response mentioned that the robot moving slowly and deeply helped the interaction be successful.
% \snnote{it'd be good to accompany this paragraph with a table} 

\subsubsection{Use of Force}
The theme of force was concerned with the amount of force the robot used during the combing interaction. The most common comment was that the robot appeared to use too much force when combing the wig, present in 15 of the responses. This was either stated generally, or quantified as the amount of movement that the mannequin head made during the combing execution. This brought up concerns for a human user's safety when using such a system in 6 of the participants' responses. Interestingly, the amount of force used was perceived as gentle and appropriate by 6 of the responses, where many cited the slower speed and more shallow combing as reasons for believing this. Participants responded that the robot did not appear to have an understanding of the sensation of touch, which worried them as the robot not realizing how hard it is pulling on knots or tangles in the hair.

\subsubsection{Characteristics of Movement}
The responses that regarded the characteristics of movement mentioned both auditory and visual components. Participants mentioned the lack of sound during the movement as uncomfortable. Visually, some participants noted the static orientation of the hand as a lack of nuance, whereas others indicated that the robot following the curves and depth of the hair as having finesse and being smooth.

% stating that the robot was not moving gracefully. The other aspect of movement  Other responses indicated that they did not believe that the robot could see very well, as it treated the hair that was close to the scalp the same as hair that was more free-floating.\snnote{is there any positive comment here?}

==> figures/content/6-Discussion.tex <==
\section{Discussion and Conclusion}

% While the results from the visual path planning study indicate that the path planning algorithm appears to work well as compared with human judgements, the results from the qualitative video study indicate that there are more considerations to take when implementing this in real-world scenarios.

% Both the results from the path evaluation and the qualitative video survey suggest that the proposed system accomplishes this hair-combing task, while following the specific style of the hair.
% \snnote{follows the hair style of a person in combing}.

Results from the qualitative survey indicate that there is more work to be done in modeling the human users and hair, for this system to be comfortable and effective for users in daily life. For example, participants indicated concern with the amount of force the robot used and that the silence of the interaction was unsettling, reflecting findings from \cite{hawkins2012informing,chen2013robots, grice2013whole,cha2015perceived}, but contrary to \cite{chen2011touched,trovato2018sound}, highlighting the importance of the task and context \cite{tennent2017good}. In addition, some participants indicated that the qualitative aspects of the robot's movement lacked nuance. Previous works have linked user perception of robot movement to the orientation and speed of the robot \cite{knight2014expressive,knight2016expressive,rond2019improv}.  For adoption and use in intended assistive services, the robot's embodiment design and affordances can be improved with best embodiment design practices, as discussed in Deng et al. \cite{deng2019embodiment}. Future work in this area should address the quality of the robot's movement, as well as other modalities of the interaction such as the sounds the robot makes as it moves through the hair and the physical design of the robot.

% \snnote{say that robot motion is important and what we have learned about the robot's motion}
% \snnote{what are design recommendations from the system?}

% This study was conducted for hairstyles with curl types ranging from 1A to 2B. This is because these hair types are most amenable to brush when dry, and their curl structure will not be as separated by repeated brush strokes, leading to unwanted frizziness. Future research is needed to address this constraint of dry hair as well as working with different hair-care products that may be used to maintain healthy hair follicles.

One limitation of this study is the use of on-line surveys, because study participants were limited to experiencing everything through only visual and auditory means. This allowed them to accurately make judgements of the sound that the robot makes while moving, but prevented them from directly experiencing tactile information such as forces used by the system. In addition, the hairstyles tested did not cover all possible hairstyles, such as very curly hair or sparse hair. Expanding the types of hairstyles that can be combed with this approach is an important direction for future work. 

% \snnote{end with implications for this work, tie this up to the bigger picture for helping users with limited mobility}
Overall, this work brings about a better understanding of how general-purpose robotic arms can effectively comb hair, adapting to different hairstyles. We presented a modular system for robotic hair combing, using a minimal setup that can work in conjunction with other assistive applications. We found that users' experience is related to the robot's movement, sound, and perceived applied force, thus opening up an exciting range of human-robot interaction research questions to which we look forward. 

%We are excited about the effects of different robot motions, sound and form can

%The evaluation of the system shows that it is able to successfully comb hair and can adapt to different hairstyles.
%In this work, we focused on the functional aspects of hair combing, the ability of the robot to make hair straighter. We contributed the design of a modular system that allows for hair combing of different hairstyles using a minimal setup that can work in conjunction with other assistive applications of the general-purpose robot arm. The evaluation of the system shows that it is able to successfully comb hair and can adapt to different hairstyles.

% The individual parts of the system can be exchanged for different implementations of the algorithms. The system is shown to effectively brush some styles of hair.

==> figures/hair__forces.tex <==
% https://repositorio.ul.pt/bitstream/10451/43338/1/MICF_Mariana_Medeiros.pdf

% This source claims that ~50N is typical for hair combing.
